One-Shot Stylization for Full-Body Human Images

The goal of human stylization is to transfer full-body human photos to a style specified by a single art character reference image. Although previous work has succeeded in example-based stylization of faces and generic scenes, full-body human stylization is a more complex domain. This work addresses several unique challenges of stylizing full-body human images. We propose a method for one-shot fine-tuning of a pose-guided human generator to preserve the "content" (garments, face, hair, pose) of the input photo and the "style" of the artistic reference. Since body shape deformation is an essential component of an art character's style, we incorporate a novel skeleton deformation module to reshape the pose of the input person and modify the DiOr pose-guided person generator to be more robust to the rescaled poses falling outside the distribution of the realistic poses that the generator is originally trained on. Several human studies verify the effectiveness of our approach.

==> content/2021_old_draft_method.tex <==
\section{Methods}
%\subsection{Recap: Dressing in Order (DIOR)}
%DiOr is a pose-conditioned person image generation pipeline which sequentially generates a person from skin to garments and thus supports tasks including pose transfer and virtual try-on. 

\section{Possible Applications}
\begin{enumerate}
    \item Try-on Fig. \ref{fig:tryon-china},\ref{fig:tryon-kon},\ref{fig:tryon-celeb},\ref{fig:tryon-frozen} 
    \item Pose transfer Fig. \ref{fig:pose-china},\ref{fig:pose-kon},\ref{fig:pose-celeb},\ref{fig:pose-mix} \textcolor{blue}{- For some cases, the art character and real person has very different skeleton ratio, maybe we should first scale the skeleton by some heuristic algorithm?}
    \item Image Translation? \ref{fig:translate} \textcolor{blue}{- If we swap all the garments and hair with the source person, can it be considered as image translation with face collapse?}
    \item Cross domain Try-on: i.e. Elsa wearing garments from old painting
    
\end{enumerate}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-chinese-tryon.pdf}
    \caption{ Try-on: Chinese Style }
    \label{fig:tryon-china}
    %\vspace*{-2pt}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-kon-tryon.pdf}
    \caption{ Try-on: Japanese Anime}
    \label{fig:tryon-kon}
    %\vspace*{-2pt}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-celeb-tryon.drawio.pdf}
    \caption{Try-on: Celebrity }
    \label{fig:tryon-celeb}
    %\vspace*{-2pt}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-frozen-try-on.drawio.pdf}
    \caption{Try-on: Frozen }
    \label{fig:tryon-frozen}
    %\vspace*{-2pt}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-chinese-pose.pdf}
    \caption{ Pose: Chinese style}
    \label{fig:pose-china}
    %\vspace*{-2pt}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-kon-pose.pdf}
    \caption{Pose: Japanese Anime}
    \label{fig:pose-kon}
    %\vspace*{-2pt}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-celeb-pose.pdf}\caption{ Pose: celebrity}
    \label{fig:pose-celeb}
    %\vspace*{-2pt}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/custom-mix-pose.pdf}\caption{ Pose: celebrity}
    \label{fig:pose-mix}
    %\vspace*{-2pt}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/custom-translate.pdf}
    \caption{Image Translation?}
    \label{fig:translate}
    %\vspace*{-2pt}
\end{figure*}

==> content/applications.tex <==
\subsection{Extensions}
By manipulating the conditioning information given to the fine-tuned generator $\mathbf{G}_a$, we can inherit the use cases of the base human generation model, such as virtual try-on and pose transfer for art characters (Fig. \ref{fig:extension}). Note, however, that the quality of pose transfer results is not very high because, as explained in Section 3.1, the training of our Dior+ generator is more heavily weighted towards reconstruction rather than pose transfer, as well as because of the obvious limitations of single-shot fine-tuning on out-of-domain data.
%We can inherit virtual try-on from the base human generation model. In Fig. \ref{fig:extension}-a the virtual try-on for a stylized person can be performed as $\mathbf{G}_{a}(I_p,\Phi'_p,g)$, where $g$ is the optional input garment. In Fig. \ref{fig:extension}-b virtual try-on for the one-shot art character can be performed as $\mathbf{G}_{a}(I_a,\Phi_a,g)$.
%\noindent \textbf{Pose Transfer} can also be achieved for the input art character as $\mathbf{G}_{a}(I_a,\Phi_{new})$, where $\Phi_{new}$ is a new pose.

\begin{figure*}
  \centering
  \includegraphics[width=0.98\textwidth]{images/stylization_mix_demo.pdf}
  \caption{Virtual Try-On.}
  \label{fig:extension}
  \vspace{-7mm}
\end{figure*}



==> content/unused_relate_work.tex <==
\section{Related Work}

\subsection{Human Stylization}
face:

full body:
\url{https://dl.acm.org/doi/pdf/10.1145/3550340.3564226}(no body scaling, not oneshot setting

\subsection{Deformable Style Transfer}
Industrial Style Transfer with Large-scale Geometric Warping and Content Preservation

\subsection{2D Person Image Generation}

Image-based person image generation tasks are popularly studied, especially for pose transfer and virtual try-on. Pose transfers models \cite{zhu2019patn,Cui_2021_dior} are usually trained on retrieval dataset Deepfashion \cite{liu2016deepfashion} and Market1501 \cite{Zheng_2015_market1501}. Both of two datasets contain large number of paired images of the same individuals to support supervised training. However, the images in such two datasets are collected in narrow domains: either well-posed model images shot in fashion studios (Deepfashion) or person crops from surveillance (Market1501), which makes the so-trained models lack robustness for outlier data and turns out a bias towards people with underrepresented race and body shape. Moreover, it is also common for such kind of models to suffer from mode collapse of person faces, i.e., the model turns to generate an average face for everyone rather than to reconstruct the face precisely for a given input person.

\subsection{3D-based Motion Transfer}
People have also studied 3D assisted person image generation, which infer 3D mesh model (SMPL\cite{}) in an intermediate stage \cite{zhao2021m3d,sarkar2020nhrr,Zakharkin_2021_pointcloudcloth}, those kinds of methods still requires a large scale of 2D and/or 3D training data and cannot be directly applied to outlier images in the wild. SPICE \cite{sanyal2021spice} is a method not requiring paired person images, but explicitly relying on 3D modeling the achieve pose transfer.

NA \cite{liu2021na} learns to do neural rendering 3D human from SMPL model and synethesize motion sequence accordingly, then can modify body shape/ratio by modifying the SMPL parameter. 

\subsection{Motion Transfer from a Single Video}
There is also a line of work learning modeling a specific individual from a single video \cite{kappel2021high}. Kappel et al. \cite{kappel2021high} learns to model an individual and transfer motions by via a model inferring body parse and body structure with 3D information as assistance. Their goal is coherent motion transfer with loose garment and it takes 3 to 4 days to train for a single video (according to their GITHUB Q/A board). 
Wang et al. \cite{wang2021dance} learns a pose-conditioned StyleGAN (512) from a single wild video which can be used for motion transfer, which takes 72 hours to train for a single video on 4 V100 GPUs.

\subsection{Person Reconstruction from Single Image}
This is a line of research learning to reconstruct a person from a single images, but their goal is 3D mesh reconstruction rather than image synthesis \cite{alldieck2019tex2shape}. 


Photo-Wakeup\cite{weng2019photowakeup} also learn to warp a 3D SMPL model for art images.

ARCH and ARCH++ \cite{he2021arch++} is a method which can do 3D reconstruction of human from a single image and used for reposing or animation generation from a graphic point of view.

Yoon et al. \cite{yoon2021pose} proposes a method reconstruct a person from a single wild image by learning a model from synethetic data to garment  semantic map and textures for new poses, in the inference stage, they represent the person by a uniform UV map and warp it back to the human in every pose. They explicitly train an inpainting model to for the novel scene and background. 
\subsubsection{Online Adaptation}
Another fewshot person generation method \cite{huang2021few} is also to build up UV map and leveraging the 3D SMPL model to render a person in different poses, which is trained from 50 videos (283k frames). After the initial training, their model can be finetuned to a specific individual by overfit the model the texture extracted from a few shots of the image of the person. However, this is a motion-focused methods, which means all the human subjects are stand far from the cermera the face is blurry by itself and hard to distinguish identity with or without finetuning?

Guan et al. \cite{guan2021bilevel} also proposes a online adaptation methods for out-of-domain data. However, their task is 3D mesh reconstruction rather than person generation.


\subsection{Fewshot Domain Adaptation for Image Generation}
